Using Case Studies to Teach Responsible AI to Industry Practitioners

Responsible AI (RAI) encompasses the science and practice of ensuring that AI design, development, and use are socially sustainable -- maximizing the benefits of technology while mitigating its risks. Industry practitioners play a crucial role in achieving the objectives of RAI, yet there is a persistent a shortage of consolidated educational resources and effective methods for teaching RAI to practitioners. In this paper, we present a stakeholder-first educational approach using interactive case studies to foster organizational and practitioner-level engagement and enhance learning about RAI. We detail our partnership with Meta, a global technology company, to co-develop and deliver RAI workshops to a diverse company audience. Assessment results show that participants found the workshops engaging and reported an improved understanding of RAI principles, along with increased motivation to apply them in their work.

==> preamble.tex <==
\usepackage[utf8]{inputenc}
\usepackage{nopageno} % remove page numbers
\usepackage{balance}  % for  \balance command ON LAST PAGE  (only there!)
\usepackage[labelfont=bf,textfont=md]{caption}
\usepackage{graphicx}
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
\usepackage{amsmath}
\usepackage{dsfont}
\usepackage{xspace}
\usepackage{color}
\usepackage{colortbl}
\usepackage{tikz}
\usepackage{microtype}
\usepackage{subfigure}

\definecolor{Gray}{gray}{0.5}
\definecolor{LightCyan}{rgb}{0.88,1,1}
\newcolumntype{a}{>{\columncolor{Gray}}c}
\def\w#1{{\cellcolor[gray]{0.5}\color{white}\textsf{#1}}}
\def\blackrow{\rowcolor[gray]{0.5}}

\newcommand*{\eg}{e.g.,\xspace}
\newcommand*{\ie}{i.e.,\xspace}
\newcommand*{\etc}{etc.\xspace}
\newcommand*{\wrt}{w.r.t.\xspace}
\newcommand*{\etal}{\emph{et~al.}\xspace}


